Identifiability, Observability, Uncertainty and Bayesian System Identification of Epidemiological Models

In this project, identifiability, observability and uncertainty properties of the deterministic and Chain Binomial stochastic SIR, SEIR and SEIAR epidemiological models are studied. Techniques for modeling overdispersion are investigated and used to compare simulated trajectories for moderately sized, homogenous populations. With the chosen model parameters overdispersion was found to have small impact, but larger impact on smaller populations and simulations closer to the initial outbreak of an epidemic. Using a software tool for model identifiability and observability (DAISY[Bellu et al. 2007]), the deterministic SIR and SEIR models was found to be structurally identifiable and observable under mild conditions, while SEIAR in general remains structurally unidentifiable and unobservable. Sequential Monte Carlo and Markov Chain Monte Carlo methods were implemented in a custom C++ library and applied to stochastic SIR, SEIR and SEIAR models in order to generate parameter distributions. With the chosen model parameters overdispersion was found to have a small impact on parameter distributions for SIR and SEIR models. For SEIAR, the algorithm did not converge around the true parameters of the deterministic model. The custom C++ library was found to be computationally efficient, and is very likely to be used in future projects.

==> Sections/Identification_Methods.tex <==
\section{Identification Methods}

\todo{Dette droppes kanskje?}
\subsection{ Linear-in-the-Parameters System with Time-varying Basis Functions}
There is an infinite number of matrices able to represent the same state-space system, making it possible to get many performance-wise good estimates which does not necessarily explain the input-output relationship of the actual system.

With measurement, state and input available, it is possible to estimate state-space models using least squares. A full (linear) state-space model is given in equation \ref{eq:subspace_method}.
\begin{align}
    Y(t) &= \begin{bmatrix}
    x(t+1)\\
    y(t)\end{bmatrix}
    ,\quad \Theta = \begin{bmatrix}
    A & B\\
    C & D\end{bmatrix} \nonumber\\
    \Phi(t) &= \begin{bmatrix}
    x(t) \\
    u(t)
    \end{bmatrix}
    ,\quad E(t) = \begin{bmatrix}
    w(t)\\
    v(t)\end{bmatrix}
    \label{eq:subspace_method}
\end{align}

The same least squares regression can be performed on nonlinear models by transforming input data to nonlinear terms, resulting in a linear-in-the-parameters state-space model. Determining the internal state of the system may not be possible, raising the need for basis functions to relate measurements to internal states.

\begin{equation}
    x(t) = L\hat{Y}(t)
\end{equation}

This is the subspace method for identifying state-space models. Since the parameters of the model may be time-varying, the subspace problem now becomes to choose basis functions for the parameters. [\cite{Italian_Model}] presents a regression model for the SIRD-model using time-varying basis functions (Equation \ref{eq:SIRD_regression_time})
\begin{align}
\begin{bmatrix} \Delta S(t)\\\Delta I(t)\\ \Delta R(t) \\ \Delta D(t)\end{bmatrix} &= \begin{bmatrix}
    -\frac{S(t)I(t)}{S(t) + I(t)}B(t) & 0 & 0\\
    \frac{S(t)I(t)}{S(t) + I(t)}B(t) & -I(t)G(t) & -I(t)M(t)\\
    0 & I(t)G(t) & 0\\
    0 & 0 & I(t)M(t)
    \end{bmatrix}
    \begin{bmatrix}
        \bs{\beta}\\
        \bs{\gamma}\\
        \bs{\nu}
    \end{bmatrix}
    \label{eq:SIRD_regression_time}
\end{align}

Where $B(t), G(t), M(t)$ are time-varying basis functions for $\bs{\beta}, \bs{\gamma}, \bs{\nu}$ respectively. While parameters are restricted to constants, the time-varying basis functions can be used to specify a wide range of changes in the model dynamics like lockdowns, periodic events and bifurcations. The resulting regression problem can be formulated as a minimization problem:



\begin{align}
\begin{split}
    S(t+1) &= -\beta \frac{S(t)I(t)}{N_{pop}}\\
    I(t+1) &= \beta \frac{S(t)I(t)}{N_{pop}} - \alpha I(t)\\
    R(t+1) &= \alpha I(t)\\
\end{split}
\end{align}
\subsection{Least Squares Methods}
\subsubsection{Linear-in-the-parameters Form}
Linear terms can be factorized from nonlinear systems to get a linear-in-the-parameters form: 
\begin{equation}
    y(k) = \sum_{i=1}^M\theta_ip_i(k) + e(k)
\end{equation}
Where $\theta_i, p_i$ are constant terms and nonlinear terms respectively, $k$ is the discrete timepoint and $e(k)$ is the total error at the timepoint. 

\begin{equation}
    \bm{Y} = P\bm{\theta} + \bm{e}
\end{equation}
Minimizing the squared sum of errors yields the nonlinear least squares solution:
\begin{align}
    S &= \zeta^T\zeta = (\bm{Y}-P\bm{\theta})^T(\bm{Y}-P\bm{\theta})
\end{align}
$\frac{dS}{d\bm{\theta}} = 0$ gives:
\begin{align}
    -2P^T\bm{Y} + 2P^TP\bm{\theta} \\
    \Longrightarrow \bm{\theta} = [P^TP]^{-1}P^T\bm{Y}
    \label{LS_sol}
\end{align}

\subsubsection{Orthogonal Version}
\label{ch:QR_decomp}

The linear-in-the-parameters form can be transformed to an orthogonal version where parameters can be determined in an uncorrelated way. The system is orthogonalized using QR-decomposition: 
\begin{equation}
    P = WA
\end{equation}
Where $W$ is upper triangular and $A$ has orthogonal columns. The Gram-Schmidt algorithm gives a perspective of how the QR-decomposition transforms the basis vectors of the system.
\begin{align}
    \begin{split}
    w_1(k) &= p_1(k)\\
    w_2(k) &= p_2(k) -proj_{w_1}p_1(k)\\
    w_3(k) &= p_3(k) - proj_{w_1}p_1(k) -proj_{w_2}p_2(k)\\
    \vdots&\\
    w_m(k) &= p_m(k) - \sum_{r=1}^{m-1}proj_{w_r}p_r(k)\\
    proj_{w_r}p_m(k) &= \frac{w_r(k)^Tp_m(k)}{w_r(k)^Tw_r(k)}
    \end{split}
\end{align}
The first basis vector of the transformed system is selected to be in the same direction as one of the systems original terms ($p_1(k)$). The following orthogonalized terms $w_i, i > 1$ are constructed by subtracting projection of the previous terms. 

With $\bm{g} = A\bm{\theta}$ it is possible to derive the least squares equation for the transformed system from equation \ref{LS_sol}:
\begin{equation}
    \bm{g} = (W^TW)^{-1}W^T\bm{y}
\end{equation}
Estimates of $y$ are retrieved directly from the transformed system:
\begin{equation}
    y = W\bm{g} + \bm{e}
\end{equation}

\subsection{FROLS Algorithm}
[\cite{billings2013nonlinear}] introduces a \textit{Forward Regression Orthogonal Least Squares} (FROLS) algorithm which proposes a solution to the ordering of terms in the QR-decomposition. The ordering of the terms can have a large impact on the number of terms needed to get consistent, accurate predictions.

\textbf{Step 1}\par
For all terms $\bm{p}$:
\begin{align}
    \bm{q}_m^{(1)} &= \bm{p}_m \\%- \sum_{r=1}^{s-1}\frac{\bm{p}_m^T\bm{q}_r}{\bm{q}_r^T\bm{q}_r}\bm{q}_r\\
    g_m^{(1)} &= \frac{\bm{y}\bm{q}_m^{(1)}}{(\bm{q}_m^{(1)})^T\bm{q}_m^{(1)}}\\
    ERR^{(1)}[m] &= (g_m^{(1)})^2[(\bm{q}_m^{(1)})^T(\bm{q}_m^{(1)})]/(\bm{y}^T\bm{y})
\end{align}

\textbf{Steg s}: $p_\ell$ is removed from the set of candidates, followed by projections of remaining candidate terms:
\begin{align}
    \bm{q}_m^{(s)} &= \bm{p}_m - \sum_{r=1}^{s-1}\frac{\bm{p}_m^T\bm{q}_r}{\bm{q}_r^T\bm{q}_r}\bm{q}_r\label{eq:sub_proj}\\
    g_m^{(s)} &= \frac{\bm{y}\bm{q}_m^{(s)}}{(\bm{q}_m^{(s)})^T\bm{q}_m^{(s)}}\\
    ERR^{(s)}[m] &= (g_m^{(s)})^2[(\bm{q}_m^{(s)})^T(\bm{q}_m^{(s)})]/\bm{y}^T\bm{y}
\end{align}
\begin{equation}
    \ell_s = \arg \max_{1\leq m\leq M}\{ERR^{(s)}[m]\}
\end{equation}
Error reduction ratios are added to a list:
\begin{equation}
    err[s] = ERR^{(s)}[\ell_s]
\end{equation}
Total ERR can be used as a termination criterion, effectively stopping the algorithm when the model performs sufficiently on training/validation-data. The predictor is constructed from the selected terms:
\begin{align}
    y(k) &= \sum_{i=1}^{M_0}g_i\bm{q}_i(k) + e(k)
    \end{align}
Similarly to the QR-decomposition this model can be transformed back to linear-in-the-parameters form with $\beta = A^{-1}\bm{g}$.
    \begin{align}
    y(k) &= \sum_{m=1}^{M_0}\beta_{\ell_m}\bm{p}_{\ell_m}(k) + e(k)
\end{align}

\subsubsection{The Volterra Series}
The Volterra series captures nonlinear dynamics in the same way as the Taylor series, but additionaly includes lagged terms which captures memory effects of the system. A Finite Impulse Response (FIR)-like Volterra model is shown in equation \ref{eq:Volterra_FIR}.
\begin{equation}
    y(k) = h_0 + h_1(1)u(k-1) + h_1(2)u(k-2) + \dots \ h_1(M)u(k-M) = h_o + \sum_{m=1}^Mh_1(m)u(k-m)
    \label{eq:Volterra_FIR}
\end{equation}

This can be extended to higher order series, resulting in the polynomial term combinations:

\begin{equation}
    y_\ell(k) = \sum_{m_1 = 1}^M \dots \sum_{m_\ell = 1}^M h_\ell(m_1,\dots,m_\ell)u(k-m_1)\dots u(k-m_\ell)
\end{equation}
Setting $M = 1$ yields multilinear terms of all possible lags in $u$ up to $m_\ell$. Increasing the order results in higher order polynomials. It should be noted that there are $\ell!$ permutations of terms $[m_1, \dots, m_\ell]$, which restricts the kernel order for practical applications. Furthermore, when recursive data is added as candidates the dimensionality of the candidate set grows even larger.

One interesting observation is the similarity between the pseudodivision algorithm used in DAISY (Section \ref{ch:pseudodiv}) and the FROLS algorithm with Volterra terms as candidate set. The pseudodivision algorithm extracts basis vectors according to a given order, leaving a polynomial remainder which is linearly uncorrelated with the extracted factor. Similarly, the FROLS algorithm extracts candidate terms and ensures that they remain linearly uncorrelated by subtracting projections (equation \ref{eq:sub_proj}).










==> Sections/Infection_Rate.tex <==
\section{Infection Rate}

